PFM-HR: Pose Flow Matching for Humanoid Robots

Motion priors improve reinforcement learning for physics-based humanoid tracking, but temporal priors require ordered motion clips, while pose priors provide limited guidance for policy-induced pose transitions. We present Pose Flow Matching for Humanoid Robots (PFM-HR), a reusable flow matching prior trained directly on large scale unordered pose data. PFM-HR introduces the Pose Geometry Score (PGS), which quantifies how joint coordinate changes during rollouts align with the local geometry of pose variation captured by the prior. Using PGS to modulate the tracking reward guides policy exploration toward structured pose changes while keeping the prior frozen across tracking tasks. Experiments demonstrate that PFM-HR improves both single motion and general motion tracking, especially for highly dynamic motions.

==> Section/Abstract.tex <==
Reinforcement learning (RL) for high-degree-of-freedom humanoid robots remains
challenging because policies must explore large continuous action spaces while
maintaining physically plausible and temporally coherent motion. Data-driven
priors can regularize this exploration, but existing motion-prior methods often
depend on trajectory-level motion data, expensive online guidance, or costly
reconstruction when new data are added. We introduce Pose Flow Matching for
Humanoid Robots (PFM-HR), a scalable pose prior for RL-based humanoid tracking.
PFM-HR trains an $x$-prediction Flow Matching model on large-scale pose data,
yielding a compact clean-pose denoising map that is reusable and efficient to
query. Although the model is trained only as a pose prior, we use its local
denoising response to provide transition-level supervision during rollout.
Specifically, we probe the frozen denoising map along rollout pose displacements
and compute a normalized Jacobian-vector response as a local transition-support
score. This score modulates the tracking reward, guiding the policy toward
transitions that are better supported by the learned pose distribution. Across challenging humanoid tracking tasks, PFM-HR improves sample efficiency
and tracking fidelity over distance-field and SDS-style prior baselines,
especially on highly dynamic motions. These results show that scalable pose
denoisers can provide effective transition-aware supervision for humanoid RL
without a separate motion prior.


==> Section/Conclusion.tex <==

\section{Conclusion}
\label{sec:conclusion}
We presented PFM-HR, a reusable Flow Matching pose prior for physics-based humanoid motion tracking that can be trained directly on large-scale unordered pose data, without pose-distance supervision or temporally segmented motion clips. Its Pose Geometry Score uses the denoiser Jacobian to evaluate whether policy-induced pose changes align with the joint co-variation patterns captured by the prior. This score can be computed efficiently through a Jacobian-vector product and used to modulate tracking rewards while keeping the prior frozen. Experiments demonstrate improved sample efficiency and tracking accuracy, particularly for dynamic and acrobatic motions, as well as compatibility with real-world humanoid deployment. 
\section{Limitations}

PFM-HR captures local co-variation in the marginal pose distribution rather
than temporal dynamics. Because the training poses are unordered and PGS is
invariant to direction reversal at a fixed query pose, it cannot assess the
likelihood or ordering of temporal transitions. Future work will explore
sign-sensitive scores and temporally conditioned priors while preserving the
efficiency and reusability of PFM-HR.

